Graph Generative Model for Benchmarking Graph Neural Networks

As the field of Graph Neural Networks (GNN) continues to grow, it experiences a corresponding increase in the need for large, real-world datasets to train and test new GNN models on challenging, realistic problems. Unfortunately, such graph datasets are often generated from online, highly privacy-restricted ecosystems, which makes research and development on these datasets hard, if not impossible. This greatly reduces the amount of benchmark graphs available to researchers, causing the field to rely only on a handful of publicly-available datasets. To address this problem, we introduce a novel graph generative model, Computation Graph Transformer (CGT) that learns and reproduces the distribution of real-world graphs in a privacy-controlled way. More specifically, CGT (1) generates effective benchmark graphs on which GNNs show similar task performance as on the source graphs, (2) scales to process large-scale graphs, (3) incorporates off-the-shelf privacy modules to guarantee end-user privacy of the generated graph. Extensive experiments across a vast body of graph generative models show that only our model can successfully generate privacy-controlled, synthetic substitutes of large-scale real-world graphs that can be effectively used to benchmark GNN models.

==> 008deprecated.tex <==
We aim to show that (1) \method scales to learn distributions of large-scale real-world graphs; (2) \method generates synthetic graphs on which GNNs perform similarly to the original graphs; (3) synthetic graphs generated by \method are sufficiently private; and (4) \method preserves distributions of graph statistics defined on the original set of computation graphs. 

\subsection{Experimental setting}
\label{sec:experiment:setting}


\textbf{Baselines:} 
We choose five state-of-the-art graph generative models that are designed to encode graph structure with node attribute information.
We extend two VAE-based graph generative models, GVAE~\citep{kipf2016variational} and GraphVAE~\citep{grover2019graphite} to generate node attributes and labels in addition to adjacency matrices from their latent variables.
We also choose three molecule graph generative models, GraphAF~\citep{shi2020graphaf}, GraphDF~\citep{luo2021graphdf}, and GraphEBM~\citep{suhail2021energy}, that do not rely on any molecule-specific traits (e.g., SMILES representation).
While GVAE encode the large-scale whole graph at once, GraphVAE, GraphAF, GraphDF, and GraphEBM are designed to receive a set of small-sized graphs (i.e., molecule graphs).
We provide the whole graph to GVAE, while provide a set of sampled computation graphs to the other baselines to fit into their design.

\textbf{Metrics:}
To measure GNN performance similarity, we run popular GNN architectures on a pair of original and synthetic graphs, then measure Mean Square Error and Pearson and Spearman correlations~\citep{myers2013research} between the resultant performance metrics on each type of graph.

Given a source graph, our method generates a set of computation graphs without any node ids. 
In other words, attackers cannot merge the generated computation graphs to restore the original graph and re-identify node information.
Thus, instead of traditional graph statistics such as orbit counts or clustering coefficients that rely on the global view of graphs, we define new graph statistics for computation graphs that are encoded by the duplicate scheme.
Duplicate scheme fixes adjacency matrices across all computation graphs by infusing structural information (originally encoded in adjacency matrices) into feature matrices.
\textit{Number of zero vectors} (corresponding to null nodes that are padded when a node has fewer neighbors than a sampling neighbor number) is inversely proportional to edge density in a computation graph.
\textit{Number of duplicate feature vectors} (which are duplicated when nodes share neighbors) is proportional to number (\#) of cycles in a computation graph, indicating how densely nodes are connected in the computation graph.

\textbf{Datasets:} We evaluate on seven public datasets --- three citation networks (Cora, Citeseer, and Pubmed)~\citep{sen2008collective}, two co-purchase graphs (Amazon Computer and Amazon Photo)~\citep{shchur2018pitfalls}, and two co-authorship graph (MS CS and MS Physic)~\citep{shchur2018pitfalls}.


\subsection{Results}
\label{sec:experiment:scalability}

\textbf{Benchmark effectiveness.} 
In Figure , we run $9$ GNN models on $7$ datasets, then plot the GNN performance on the original graphs and generated graphs by each baseline.
The ideal benchmark would be plotted as $x=y$ (blue line in Figure).
As shown in Figure, GNN performance on graphs generated by our method preserves the original trend effectively, closely located to $x=y$.
The Figure shows the MSE between GNN performance on original and synthetic graphs.
All baselines fail to encode the graph structure properly.
None of them is originally designed to generate node attributes with adjacency matrix.
Also GraphAF, GraphDF, GraphEBM are designed to process the small-scale graphs with a few number of integer-valued attributes, failed to encode the large-scale graphs.

\textbf{Graph statistics.}
For fair comparison, for generated computation graphs by each baseline, we duplicate-encode them and compute the two proxy graph statistics, number of zero vectors and duplicate vectors in each computation graphs.
In Figure, we plot the distributions of this two statistics generated by each baseline.


\textbf{Scalability.}


\textbf{Privacy.}
We examine the performance-privacy trade-off across different privacy guarantees.
For $k$-anonymity, we use the k-means clustering algorithm~\citep{bradley2000constrained} varying the minimum cluster size $k$.
For Differential Privacy (DP) for node attributes, we use DP k-means~\citep{chang2021locally} varying the privacy cost $\epsilon$ while setting $\delta=0.01$.
As expected, in Table~\ref{tab:privacy_summary}, higher $k$ and smaller $\epsilon$ (i.e., stronger privacy) hinder the generative model's ability to learn the exact distributions of the original graphs, and the GNN performance gaps between original and generated graphs increase (lower Pearson and Spearman coefficients).
Detailed GNN accuracies could be found in Table~\ref{tab:appendix:privacy} in Appendix~\ref{appendix:privacy}.
To provide DP for edge distributions, we use DP stochastic gradient descent~\citep{song2013stochastic} to train the transformer, varying the privacy cost $\epsilon$ while setting $\delta=0.1$.
In Table~\ref{tab:privacy_summary}, even with astronomically low privacy cost ($\epsilon=10^6$), the performance of our generative model degrades significantly.
When we set $\epsilon=10^9$ (which is impractical), we can finally see a reasonable performance.
This shows the limited performance of DP SGD on the transformer architecture.


To the best of our knowledge, no other generic graph generative model was designed to output a triad of the adjacency matrix, node attribute matrix, and node labels.
We extend two VAE-based graph generative models, GVAE~\citep{kipf2016variational} and Graphite~\citep{grover2019graphite} to generate node attributes and labels in addition to adjacency matrices from their latent variables.
We also choose three molecule graph generative models, GraphAF~\citep{shi2020graphaf}, GraphDF~\citep{luo2021graphdf}, and GraphEBM~\citep{suhail2021energy}, that do not rely on any molecule-specific traits (e.g., SMILES representation). GraphAF, GraphDF, and Graphite meet out-of-memory errors on even the smallest dataset, Cora (Table~\ref{tab:appendix:scalablity}in Appendix~\ref{appendix:scalability}).
This is not surprising, given they were originally designed for small-size molecule graphs.
The remaining baselines (GVAE and GraphEBM), however, fail to learn any meaningful node attribute/label distributions from the original graphs.
For instance, the predicted distribution sometimes collapses to generating the the same node feature/labels across all nodes, which is obviously not the most effective benchmark ($100\%$ accuracy for all GNN models).
We show their results and our analysis in the Appendix~\ref{appendix:scalability}.
Only our method can successfully generate benchmark graphs across all datasets with meaningful node attribute/label distributions (Tables~\ref{tab:nc_example} and~\ref{tab:nc_summary}).

\begin{table*}[]
    \caption{
    \small
	\textbf{GNN performance on original and generated graphs in three different scenarios with three variations.}
	\# NE denotes number of noise edges and $\alpha$ denotes the PPR coefficient used for distribution shift.
	}
	\label{tab:nc_example}
	\centering
    \tiny
\begin{tabular}{clcc|clcc|clcc} \toprule\hline
\multicolumn{4}{c|}{\textbf{Aggregation with noise (Citeseer)}}                                                                 & \multicolumn{4}{c|}{\textbf{Sampling with noise (Amazon Photo)}}                                                                       & \multicolumn{4}{c}{\textbf{Distribution shift (MS Physic)}}                                                                        \\ \hline
\multicolumn{1}{c|}{\textbf{\#NE}}               & \multicolumn{1}{c|}{\textbf{model}} & \textbf{Original} & \textbf{Generated} & \multicolumn{1}{c|}{\textbf{\#NE}}               & \multicolumn{1}{c|}{\textbf{model}}   & \textbf{Original} & \textbf{Generated} & \multicolumn{1}{c|}{\textbf{$\alpha$}}                 & \multicolumn{1}{c|}{\textbf{model}} & \textbf{Original} & \textbf{Generated} \\ \hline\midrule
\multicolumn{1}{c|}{\multirow{4}{*}{\textbf{0}}} & \multicolumn{1}{l|}{\textbf{GCN}}   & 0.73+0.004        & 0.59+0.024         & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{0}}} & \multicolumn{1}{l|}{\textbf{GSage}}   & 0.75+0.009        & 0.53+0.028         & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{iid}}}  & \multicolumn{1}{l|}{\textbf{GSage}} & 0.93+0.002        & 0.84+0.008         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{SGC}}   & 0.73+0.002        & 0.58+0.029         & \multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{AS-GCN}}  & 0.14+0.016        & 0.12+0.020         & \multicolumn{1}{c|}{}                               & \multicolumn{1}{l|}{\textbf{SGC}}   & 0.92+0.001        & 0.84+0.007         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{GIN}}   & 0.71+0.009        & 0.57+0.028         & \multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{FastGCN}} & 0.92+0.004        & 0.87+0.002         & \multicolumn{1}{c|}{}                               & \multicolumn{1}{l|}{\textbf{GAT}}   & 0.93+0.002        & 0.82+0.011         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{GAT}}   & 0.71+0.003        & 0.57+0.029         & \multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{PASS}}    & 0.85+0.011        & 0.54+0.049         & \multicolumn{1}{c|}{}                               & \multicolumn{1}{l|}{\textbf{PPNP}}  & 0.93+0.005        & 0.84+0.007         \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\textbf{2}}} & \multicolumn{1}{l|}{\textbf{GCN}}   & 0.57+0.005        & 0.46+0.013         & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{2}}} & \multicolumn{1}{l|}{\textbf{GSage}}   & 0.40+0.012        & 0.36+0.009         & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{0.01}}} & \multicolumn{1}{l|}{\textbf{GSage}} & 0.83+0.033        & 0.76+0.019         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{SGC}}   & 0.57+0.005        & 0.47+0.019         & \multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{AS-GCN}}  & 0.12+0.014        & 0.11+0.027         & \multicolumn{1}{c|}{}                               & \multicolumn{1}{l|}{\textbf{SGC}}   & 0.84+0.004        & 0.74+0.015         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{GIN}}   & 0.54+0.020        & 0.44+0.015         & \multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{FastGCN}} & 0.87+0.005        & 0.81+0.010         & \multicolumn{1}{c|}{}                               & \multicolumn{1}{l|}{\textbf{GAT}}   & 0.87+0.007        & 0.78+0.009         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{GAT}}   & 0.57+0.014        & 0.44+0.010         & \multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{PASS}}    & 0.73+0.018        & 0.59+0.011         & \multicolumn{1}{c|}{}                               & \multicolumn{1}{l|}{\textbf{PPNP}}  & 0.84+0.007        & 0.74+0.009         \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\textbf{4}}} & \multicolumn{1}{l|}{\textbf{GCN}}   & 0.51+0.027        & 0.41+0.003         & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{4}}} & \multicolumn{1}{l|}{\textbf{GSage}}   & 0.26+0.009        & 0.20+0.014         & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{0.3}}}  & \multicolumn{1}{l|}{\textbf{GSage}} & 0.84+0.012        & 0.68+0.023         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{SGC}}   & 0.52+0.009        & 0.41+0.005         & \multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{AS-GCN}}  & 0.10+0.025        & 0.13+0.054         & \multicolumn{1}{c|}{}                               & \multicolumn{1}{l|}{\textbf{SGC}}   & 0.81+0.009        & 0.70+0.009         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{GIN}}   & 0.48+0.023        & 0.41+0.007         & \multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{FastGCN}} & 0.67+0.003        & 0.62+0.006         & \multicolumn{1}{c|}{}                               & \multicolumn{1}{l|}{\textbf{GAT}}   & 0.85+0.011        & 0.72+0.019         \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{GAT}}   & 0.49+0.012        & 0.40+0.009         & \multicolumn{1}{c|}{}                            & \multicolumn{1}{l|}{\textbf{PASS}}    & 0.64+0.017        & 0.50+0.017         & \multicolumn{1}{c|}{}                               & \multicolumn{1}{l|}{\textbf{PPNP}}  & 0.81+0.012        & 0.70+0.009         \\ \hline
\multicolumn{2}{c|}{\textbf{Pearson / Spearman}}                                       & \multicolumn{2}{c|}{0.991 / 0.964}     & \multicolumn{2}{c|}{}                                                                    & \multicolumn{2}{c|}{0.958 / 0.916}     & \multicolumn{2}{c|}{}                                                                     & \multicolumn{2}{c}{0.925 / 0.815}     \\\hline\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[]
    \caption{
    \small
	\textbf{Benchmark effectiveness on node classification.}
	Pearson and Spearman scores measure the correlation in ranking of GNN models on original and generated graphs; a score of $1$ denotes perfect correlation.
	}
	\label{tab:nc_summary}
	\centering
    \tiny
\begin{tabular}{l|cc|cc|cc|cc}\toprule\hline
                   & \multicolumn{2}{c|}{\textbf{Aggregation with noise}} & \multicolumn{2}{c|}{\textbf{Sampling with noise}} & \multicolumn{2}{c|}{\textbf{Sampling number}} & \multicolumn{2}{c}{\textbf{Distribution shift}} \\
\textbf{Dataset}   & \textbf{Pearson}         & \textbf{Spearman}         & \textbf{Pearson}        & \textbf{Spearman}       & \textbf{Pearson}      & \textbf{Spearman}     & \textbf{Pearson}       & \textbf{Spearman}      \\ \midrule\hline
\textbf{Cora}      & 0.934                    & 0.950                     & 0.943                   & 0.894                   & 0.967                 & 0.814                 & 0.867                  & 0.833                  \\
\textbf{Citeseer}  & 0.991                    & 0.964                     & 0.955                   & 0.977                   & 0.973                 & 0.904                 & 0.812                  & 0.799                  \\
\textbf{Pubmed}    & 0.818                    & 0.791                     & 0.900                   & 0.867                   & 0.989                 & 0.824                 & 0.830                  & 0.794                  \\
\textbf{Amazon Computer}   & 0.825                    & 0.778                     & 0.885                   & 0.916                   & 0.975                 & 0.890                      & 0.906                  & 0.860                  \\
\textbf{Amazon Photo}   & 0.918                    & 0.893                     & 0.958                   &  0.916                       & 0.961                 & 0.931                 & 0.771                  & 0.847                  \\
\textbf{MS CS}     & 0.916                    & 0.922                     & 0.974                   &    0.956                     & 0.986                 & 0.901                 & 0.792                  & 0.751                  \\
\textbf{MS Physic} & 0.661                    & 0.685                     & 0.956                   & 0.951                        & 0.947                 & 0.901                      & 0.925                  & 0.815 \\ \hline\bottomrule                
\end{tabular}
\vspace{2mm}
\end{table*}

\vspace{-2mm}
\subsection{Benchmark effectiveness}
\label{sec:experiment:benchmark}

To examine the benchmark effectiveness of our generative model, we design $4$ different scenarios where the performance of different GNN architectures varies widely.
In each scenario, we provide $3$ variations to graphs and run $4$ GNN models on each variation.
For each scenario-variation, we report Pearson and Spearman correlations of the GNN performance metrics on the original graph against those on the generated graph.
Due to the space limitation, we present detailed GNN accuracies only on a few datasets/scenarios in Table~\ref{tab:nc_example}.
Results on other datasets can be found in Appendix~\ref{appendix:benchmark}.
Note that Table~\ref{tab:nc_summary} presents the correlation coefficients across all datasets and scenarios. 
Descriptions of each GNN model can be found in the Appendix~\ref{appendix:gcn:models}.

\paragraph{SCENARIO 1: noisy edges on aggregation strategies.}
We choose four different GNN models with different aggregation strategies: GCN~\citep{kipf2016semi} with mean aggregator, GIN~\citep{xu2018powerful} with sum aggregator, SGC~\citep{wu2019simplifying} with linear aggregator, and GAT~\citep{velivckovic2017graph} with attention aggregator.
Then we modify the graph by adding different numbers of noisy edges (randomly connected with any node in the graph) to each node and check how the GNN performance changes.
In Table~\ref{tab:nc_example}, first three columns show the result in the Citeseer dataset.
When more noisy edges are added, the accuracy across all GNN models drops in the original graphs.
These trends can be nearly exactly captured in GNN performance on the generated graphs (both Pearson and Spearman correlation rates are up to $0.964$).
This shows that the synthetic graphs generated by our method successfully capture the noisy edge distributions introduced in the original graphs.

\paragraph{SCENARIO 2: noisy edges on neighbor sampling.}
We choose four different GNN models with different neighbor sampling strategies: GraphSage (abbreviated as GSage in Table~\ref{tab:nc_example})~\citep{hamilton2017inductive} with random sampling, FastGCN~\citep{chen2018fastgcn} with heuristic layer-wise sampling, AS-GCN~\citep{huang2018adaptive} with trainable layer-wise sampling, and PASS~\citep{yoon2021performance} with trainable node-wise sampling.
We then add noisy edges as described in the ENV 1 and check how the different sampling policies deal with noisy neighbors.
In Table~\ref{tab:nc_example}, FastGCN shows highest accuracies across different number of nosiy edges, followed by PASS, GraphSage, and AS-GCN on the original graphs on the Amazon Photo dataset; and this trend is well-preserved on the generated graphs, showing $0.958$ Pearson correlation.

\begin{wraptable}{r}{0.47\textwidth}
\vspace{-7mm}
\caption{
    \small
	\textbf{Benchmark effectiveness and GNN performance on link prediction.}
	}
	\label{tab:lp_summary}
	\centering
    \tiny
\begin{tabular}{l|l|l|c|c}\toprule\hline
\textbf{Dataset}                   & \multicolumn{1}{c|}{\textbf{Pearson}} & \multicolumn{1}{c|}{\textbf{Spearman}} & \textbf{Pearson}       & \textbf{Spearman}      \\ \hline
\textbf{Cora}                      & \multicolumn{1}{c|}{0.781}            & \multicolumn{1}{c|}{0.741}             & \multirow{5}{*}{0.742} & \multirow{5}{*}{0.754} \\
\textbf{Citeseer}                  & \multicolumn{1}{c|}{0.808}            & \multicolumn{1}{c|}{0.824}             &                        &                        \\
\textbf{Pubmed}                    & \multicolumn{1}{c|}{0.725}            & \multicolumn{1}{c|}{0.420}             &                        &                        \\
\textbf{AmazonC}                   & \multicolumn{1}{c|}{0.652}            & \multicolumn{1}{c|}{0.559}             &                        &                        \\
\textbf{AmazonP}                   & \multicolumn{1}{c|}{0.887}            & \multicolumn{1}{c|}{0.443}             &                        &                        \\ \hline\bottomrule \toprule
\textbf{Dataset}                   & \textbf{Predictor}                    & \textbf{Model}                         & \textbf{Original}      & \textbf{Generated}     \\ \hline
\multirow{8}{*}{\textbf{Citesser}} & \multirow{4}{*}{\textbf{Dot}}         & \textbf{GCN}                           & 0.69+0.007             & 0.65+0.026             \\
                                   &                                       & \textbf{SGC}                           & 0.70+0.003             & 0.67+0.022             \\
                                   &                                       & \textbf{GIN}                           & 0.83+0.008             & 0.65+0.010             \\
                                   &                                       & \textbf{GAT}                           & 0.75+0.005             & 0.68+0.021             \\ \cline{2-5} 
                                   & \multirow{4}{*}{\textbf{MLP}}         & \textbf{GCN}                           & 0.58+0.005             & 0.59+0.010             \\
                                   &                                       & \textbf{SGC}                           & 0.58+0.008             & 0.59+0.023             \\
                                   &                                       & \textbf{GIN}                           & 0.57+0.011             & 0.61+0.024             \\
                                   &                                       & \textbf{GAT}                           & 0.61+0.005             & 0.62+0.009            \\\hline\bottomrule
\end{tabular}
\vspace{-7mm}
\end{wraptable}

\paragraph{SCENARIO 3: different sampling numbers on neighbor sampling.}
We choose the same four GNN models with different neighbor sampling strategies as in EV2.
Then we change the number of sampled neighbor nodes and check how the GNN performance is affected.
As shown in Table~\ref{tab:nc_summary}, trends among original graphs --- more neighbors are sampled, GNN performance generally increases --- are successfully captured in the generated graphs with $0.991$ and $0.931$ Pearson and Spearman correlations, respectively, across all datasets.
You can find the detailed GNN accuracies in Appendix~\ref{appendix:benchmark}.

\paragraph{SCENARIO 4: distribution shift.}
~\citep{zhu2021shift} proposed a biased training set sampler to examine each GNN model's robustness to distribution shift between the training/test time.
The biased sampler picks a few seed nodes and finds nearby nodes using the Personalized PageRank vectors~\citep{page1999pagerank} $\pi_{\text{ppr}} = (I - (1-\alpha)\Tilde{A})^{-1}$ with decaying coefficient $\alpha$, then uses them to compose a biased training set.
We choose the same GNN models, GCN~\citep{kipf2016semi}, SGC~\citep{wu2019simplifying}, GAT~\citep{velivckovic2017graph}, and PPNP~\citep{klicpera2018predict}, as the original paper~\citep{zhu2021shift} chose for their baselines.
We vary $\alpha$ and check how each GNN models deal with the biased training set.
In the last three columns in Table~\ref{tab:nc_example}, the performance of GNN models drops as $\alpha$ increases, and the generated graphs successfully capture these trends.

\paragraph{Link prediction.}
As nodes are the minimum unit in graphs that compose edges or subgraphs, we can generate subgraphs for edges by merging computation graphs of their component nodes. 
Here we show link prediction results on original graphs are also preserved successfully on our generated graphs.  
We run GCN, SGC, GIN, and GAT on graphs, followed by Dot product or MLP to predict link probabilities. 
Table~\ref{tab:lp_summary} shows Pearson and Spearman correlations across 8 different combinations of link prediction models ($4$ GNN models $\times$ $2$ predictors) on each dataset and across the whole datasets.
The lower table shows the detailed link prediction accuracies on the Citeseer dataset. 
Our model generates graphs that substitute original graphs successfully, preserving the ranking of GNN link prediction performance with $0.754$ Spearman correlation across the datasets.

\begin{table*}[h]
    \caption
    {
        \small
	    \textbf{Privacy-Performance trade-off in graph generation on the Cora dataset}
	}
	\label{tab:privacy_summary}
	\centering
    \tiny
\begin{tabular}{l|c|c|ccc|ccc|cc}\toprule\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{}}} & \multirow{2}{*}{\textbf{Original}} & \multirow{2}{*}{\textbf{No privacy}} & \multicolumn{3}{c|}{\textbf{K-anonymity}}         & \multicolumn{3}{c|}{\textbf{DP kmean ($\delta = 0.01$)}} & \multicolumn{2}{c}{\textbf{DP SGD ($\delta = 0.1$)}} \\
\multicolumn{1}{c|}{}                           &                                    &                                      & \textbf{$k=100$} & \textbf{$k=500$} & \textbf{$k=1000$} & \textbf{$\epsilon = 1$}  & \textbf{$\epsilon = 10$}  & \textbf{$\epsilon = 25$}  & \textbf{$\epsilon = 10^6$}       & \textbf{$\epsilon = 10^9$}      \\ \hline\midrule
\textbf{Pearson}                                & 1.000                              & 0.934                                & 0.916          & 0.862          & 0.030           & 0.874           & 0.844            & 0.804            & 0.112                   & 0.890                   \\
\textbf{Spearman}                               & 1.000                              & 0.935                                & 0.947          & 0.812          & 0.018           & 0.869           & 0.805            & 0.807            & 0.116                   & 0.959   \\ \hline\bottomrule               
\end{tabular}
\end{table*}



\begin{figure*}[t!]
 	\centering
 	\includegraphics[width=0.6\linewidth]{FIG/statistics_legend.png}
 	\subfigure[\small\# zero vectors on each computation graph]
 	{
 	\label{fig:statistics:zeros}
 	\includegraphics[width=.48\linewidth]{FIG/statistics_zeros.png}
 	}
 	\subfigure[\small\# redundant vectors on each computation graph]
 	{
 	\label{fig:statistics:dups}
 	\includegraphics[width=.48\linewidth]{FIG/statistics_dups.png}
 	}
 	\caption
 	{   
 	    \small
 	    \textbf{\method preserves distributions of graph statistics in generated graphs for each dataset:} Duplicate encoding infuses graph structure into feature matrices of computation graphs. In each computation graph, \# zero vectors is inversely proportional to edge density, while \# redundant vectors is proportional to \# cycles.
 	}
 	\label{fig:statistics}
 	\vspace{2mm}
 \end{figure*}

% \subsection{Graph statistics}
% \label{sec:experiment:statistics}

% Given a source graph, our method generates a set of computation graphs without any node ids. 
% In other words, attackers cannot merge the generated computation graphs to restore the original graph and re-identify node information.
% Thus, instead of traditional graph statistics such as orbit counts or clustering coefficients that rely on the global view of graphs, we define new graph statistics for computation graphs that are encoded by the duplicate scheme.
% Duplicate scheme fixes adjacency matrices across all computation graphs by infusing structural information (originally encoded in adjacency matrices) into feature matrices.
% \textit{Number of zero vectors} (corresponding to null nodes that are padded when a node has fewer neighbors than a sampling neighbor number) is inversely proportional to edge density in a computation graph.
% \textit{Number of duplicate feature vectors} (which are duplicated when nodes share neighbors) is proportional to number (\#) of cycles in a computation graph, indicating how densely nodes are connected in the computation graph.
% In Figure~\ref{fig:statistics}, we present distributions of a) number of zero vectors and b) number of redundant vectors each computation graph has on each dataset.
% Five different datasets show distinct distributions on these two statistics, and distributions of both statistics are well preserved in generated graphs.
% For instance, in Figure~\ref{fig:statistics:zeros}, green lines (Pubmed) are lower than purple and red lines (Amazon Computer and Amazon Photo) at the beginning and become higher in both plots.
% In Figure~\ref{fig:statistics:dups}, purple lines (Amazon Computer) are slightly higher than red lines (Amazon Photo) until $x=300$, then become lower in both plots.
% In the same figure, blue, yellow, and green lines (Cora, Citeseer, and Pubmed) decrease sharply compared to purple and red lines (Amazon Computer and Amazon Photo) in both plots.
% This shows our generative model preserves graph structures encoded in feature matrices successfully.

\subsection{Scalability issues on baseline generative models}
\label{appendix:scalability}

In Table~\ref{tab:appendix:scalablity}, GraphAF~\citep{shi2020graphaf}, GraphDF~\citep{luo2021graphdf}, and Graphite~\citep{grover2019graphite} meet out-of-memory errors on both the Cora and Citeseer datasets.
This is because they were originally designed for small-size molecule graphs.
The remaining baselines, GVAE~\citep{kipf2016variational} and GraphEBM~\citep{suhail2021energy} successfully generate graphs, however, fail to learn any meaningful node attribute/label distributions from the original graphs.
Especially, GraphEBM generates graphs whose distribution collapses to generating the the same node feature/labels across all nodes, showing $100\%$ accuracy for all GNN models, which is obviously not the most effective benchmark.
Note that none of existing graph generative models is designed for GNN benchmarking --- simultaneous generation of adjacency, node feature, and node label matrices, rather they all focus only on the generation of adjacency matrices.
This result shows the tricky aspects of graph generation and relations among
graph structure, node attributes and labels, and a large room for improvement in the graph generation field.

==> check_list.tex <==
\begin{enumerate}

\item For all authors...
\begin{enumerate}
    \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
    \item Did you describe the limitations of your work?
    \answerYes{We mention it in Section~\ref{sec:conclusion}.}
    \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We mention about possible private information leakage in graph data sharing in Section~\ref{sec:introduction}. By proposing a novel graph generative model with privacy guarantees, we can alleviate this issue.}
    \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
    \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{We mention the full set of assumptions for Claims 1,2, and 3 in Section~\ref{sec:proposed_method:analysis}.}
    \item Did you include complete proofs of all theoretical results?
    \answerNA{The proof for Claims 1,2, and 3 is described in Appendix.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
    \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{They are all included in the supplemental material.}
    \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{They are all described in Appendix.}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{They are all described in Tables~\ref{tab:aggregation},~\ref{tab:sampling} and~\ref{tab:sampling2}.}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{They are all described in Appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
    \item If your work uses existing assets, did you cite the creators?
    \answerYes{We used an open source library DIG for graph generative models and we cited them in Appendix.}
    \item Did you mention the license of the assets?
    \answerNA{They are all public libraries.}
    \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We include our code in the supplemental material.}
    \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We do not use any personal data.}
    \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We do not use any personal data.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
    \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
    \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
    \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

